ICPR 2024 Competition on Multilingual Claim-Span Identification

A lot of claims are made in social media posts, which may contain misinformation or fake news. Hence, it is crucial to identify claims as a first step towards claim verification. Given the huge number of social media posts, the task of identifying claims needs to be automated. This competition deals with the task of 'Claim Span Identification' in which, given a text, parts / spans that correspond to claims are to be identified. This task is more challenging than the traditional binary classification of text into claim or not-claim, and requires state-of-the-art methods in Pattern Recognition, Natural Language Processing and Machine Learning. For this competition, we used a newly developed dataset called HECSI containing about 8K posts in English and about 8K posts in Hindi with claim-spans marked by human annotators. This paper gives an overview of the competition, and the solutions developed by the participating teams.

==> sections/logistics.tex <==
%\section{Tentative Schedule and Expected Participants}


\begin{table}[tb]
\centering
\small
\begin{tabular}{|c|p{0.85\textwidth}|}
\hline
\textbf{Apr 18} & Competition website goes live. Training and Validation data released \\
\hline
\textbf{Jul 10} & Test data released \\
\textbf{Jul 21} & Deadline for competition participants (to submit predictions on test data)\\
\textbf{Aug 11}  & Results declared (based on performance on test data)\\
\hline
\textbf{Aug 18} & Deadline for initial submission of competition reports \\
\textbf{Sep 02} & Camera-ready papers due \\
\textbf{Oct 28} & Communicate winners to Chairs \\
\hline
\textbf{Dec 1-5} & Presentation at ICPR Conference \\
\hline
\end{tabular}
\vspace{2mm}
\caption{Tentative schedule for the competition}
\vspace*{-5mm}
\label{tag:schedule}
\end{table}



\section{Competition Organizers}

\begin{itemize}
\item \textbf{\large Soham Poddar} (\url{https://sohampoddar26.github.io/}) \\
    \textbf{\textit{Email:}} sohampoddar@kgpian.iitkgp.ac.in
    \vspace{1mm}
    
    \noindent \textit{Soham Poddar is a senior PhD Scholar in the Department of Computer Science and Engineering at Indian Institute of Technology, Kharagpur. His research areas include social media analytics and natural language processing. His work has been published in reputed conferences and journals like ACM SIGIR, AAAI ICWSM, ACM Tranactions on the Web and AACL-IJCNLP. He has experience of organizing several shared tasks / competitions at the FIRE conference.}\\
    

\item \textbf{\large Biswajit Paul} \\
\textbf{\textit{Email:}} biswajit.cair@gov.in 
    \vspace{1mm}
    
\textit{Biswajit Paul is Scientist (F) at the Centre for Artificial Intelligence and Robotics(CAIR), Defence Research \& Development Organisation at Bangalore, India. His research interests are in Natural Language Processing, focusing on Machine Translation, Knowledge harvesting from web and Low resource NLP. 
He presently leads the Computational Linguistics team that focuses on R\&D of NLP technologies for the Indian Defence. Some of his works are published in WMT, SemEval, WAT etc. He is also member of many review committees for DRDO projects with academia and industries.} \\

\item \textbf{\large Moumita Basu} (\url{https://amitykolkata.irins.org/profile/376094}) \\
    \textbf{\textit{Email:}} mbasu@kol.amity.edu
    \vspace{1mm}

\textit{Moumita Basu is an Associate Professor at the Department of Computer Science and Engineering, Amity University Kolkata. Her research interests are in Social Media analysis in the domain of Disaster Management and Transportation. Her research is interdisciplinary and uses techniques from Machine Learning, Deep Learning, and Natural Language Processing.  
She has several publications in esteemed journals and refereed conferences. She received her PhD in Computer Science from Indian Institute of Engineering Science and Technology Shibpur in 2021. She has prior experience of organizing Data Challenges successfully with FIRE Conference in the years 2017, 2018 and 2021 and 2023 as a track chair.} \\

\item \textbf{\large Saptarshi Ghosh} (\url{http://cse.iitkgp.ac.in/$\sim$ saptarshi/})\\
    \textbf{\textit{Email:}} saptarshi@cse.iitkgp.ac.in
    \vspace{1mm}

    \textit{Saptarshi Ghosh is an Associate Professor at the Department of Computer Science and Engineering, Indian Institute of Technology Kharagpur. His research interests include Legal Analytics, Social Network Analysis, and Algorithmic Bias and Fairness. He has published more than 100 research papers in reputed conferences and journals -- including WWW, SIGIR, EMNLP, ICWSM, CSCW, ACM Transactions on the Web, IEEE Transactions on Computational Social Systems -- and has investigated more than 10 research projects sponsored by the Government of India and various industries. He presently leads a Max Planck Partner Group that focuses on topics related to Algorithmic bias and fairness. He has organized several data challenges / competitions, notably with the Forum for Information Retrieval (FIRE) conferences.}    
\end{itemize}

\vspace*{2mm}
\noindent Note that the organizers have prior experience in organizing several data challenges / shared tasks with the Forum for Information Retrieval (FIRE) conferences. 
These include the data challenge track ``Artificial Intelligence on Social Media''\footnote{\url{https://sites.google.com/view/aisome/aisome}} with FIRE 2023, and the ``Information Retrieval from Microblogs during Disasters'' track with FIRE2022\footnote{\url{https://sites.google.com/view/irmidis-fire2022/irmidis}}, FIRE2021, FIRE2018, etc.  
